When Safety Speaks a Language: A Mechanistic Analysis of Safety-Language Identity Entanglement in LLMs

Safety alignment of large language models (LLMs) degrades across languages, yet the internal mechanism driving this asymmetry remains poorly understood. Our work, therefore, presents a systematic mechanistic analysis of multilingual safety using sparse autoencoder (SAE) features, sparse interpretable directions in the residual stream associated with harmful and harmless model behavior across three instruction-tuned LLMs, eight languages, and all model layers. We observe that safety-relevant features are architecture-dependent in terms of where they are located and how they are distributed across layers. Additionally, they are geometrically entangled with language identity and exhibit cross-lingual sharing patterns, i.e., languages share safety features to varying degrees across model depths and architectures. This safety-language entanglement has direct consequences such that ablating safety features impacts not only harmful response rates but also target language, with the degree of intervention predicted by the relationship between safety and language features. Our findings qualify the language-universality of safety alignment as architecture-dependent and offer a mechanistic account of multilingual safety interventions.

==> sections/results_old.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_normalised_peaks.png}
\caption{
    Normalised peak layer positions (as \% of total model depth) for harm (red) and harmless (blue) signals across 8 languages and 3 LLMs (circle=Llama, square=Qwen, triangle=Gemma). The dashed line marks the approximate late-phase onset ($\sim$68\% depth).
}
\label{fig:rq1_peaks}\paragraph{Language Identity Preservation.}
\end{figure*}



\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_llama.png}
\caption{
    Harm (red, solid) and harmless (blue, dashed) MI signal strength across layers for all languages 
    (AR, EN, HI, VI) across Llama. Dotted vertical lines mark phase boundaries (E=early, M=middle, L=late). Filled markers indicate peak layers; shaded region shows the gap between harm and harmless peaks.
}
\label{fig:rq1_signal_llama}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_qwen.png}
\caption{
    Harm (red, solid) and harmless (blue, dashed) MI signal strength across layers for all languages 
    (AR, EN, HI, VI) across Qwen. Dotted vertical lines mark phase boundaries (E=early, M=middle, L=late). Filled markers indicate peak layers; shaded region shows the gap between harm and harmless peaks.
}
\label{fig:rq1_signal_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_gemma.png}
\caption{
    Harm (red, solid) and harmless (blue, dashed) MI signal strength across layers for all languages 
    (AR, EN, HI, VI) across Gemma. Dotted vertical lines mark phase boundaries (E=early, M=middle, L=late). Filled markers indicate peak layers; shaded region shows the gap between harm and harmless peaks.
}
\label{fig:rq1_signal_gemma}
\end{figure*}


\subsection{RQ1: Layer-wise distribution of harm and harmless signals in LLMs across languages} 
We analyze layer-wise mutual information (MI) scores for top-5 harm and harmless features across 32 layers (Llama), 28 layers (Qwen), and 42 layers (Gemma) for all 8 languages. We then identify peak layers for each signal and characterize the gap between harm and harmless peaks as a measure of circuit asymmetry. Table 1 summarizes peak layers across languages and models. 

\par \noindent \textbf{Early layers show universal signal absence.} Across LLMs and all 8 languages, early layers (Llama L0–L10, Qwen L0–L9, Gemma L0–L13) show near-zero MI scores for both harm and harmless features (Figures \ref{fig:rq1_signal_llama} - \ref{fig:rq1_signal_gemma}). This uniIn Gemma, both metrics collapse below model average 
(harm decoder mean $z = -0.545$) with 6/8 languages 
showing Jaccard $0.000$, yet decoder remains non-zero 
($0.077$--$0.129$).
This reveals a fundamental divergence: Llama and Qwen 
couple harm-detection to language identity in late 
layers where safety is strongest, while Gemma 
decouples safety signal strength from language 
entanglement entirely (Appendix~\ref{app:rq2_late} 
for per-language details).versal absence indicates that safety computation does not occur during surface-level feature extraction in early layers, holding across architectures of different depth and training procedures.

\par \noindent \textbf{Middle layers diverge across architectures.} Llama shows three languages with middle-layer peaks: EN harm signal at L19, DE harmless signal at L18, and VI harmless signal at L14; the earliest safety-relevant signal observed across LLMs (Figure \ref{fig:rq1_signal_llama} and Table \ref{tab:rq1_peak_layers}). However, Qwen and Gemma show complete absence of middle-layer peaks across all 8 languages, deferring all safety computation to late layers (Figures \ref{fig:rq1_signal_qwen} and \ref{fig:rq1_signal_gemma}). %Since Qwen (28L) and Gemma (42L) differ substantially in depth yet  both show zero middle-layer peaks, this divergence from Llama  reflects differences in safety alignment methodology rather than model depth.

%This divergence across models of different depths (28 vs 42 layers) reflects differences in safety alignment methodology rather than model depth.

\par \noindent \textbf{Late layers are the dominant location for 
safety computation, with model-dependent ordering of harm and 
harmless signals.} As shown in Table~\ref{tab:rq1_peak_layers} and Figure \ref{fig:rq1_peaks}, both harm and harmless signal peaks concentrate in late layers across all three models, with progressive exclusivity: Llama shows 5/8 languages with both signals in late layers (3 languages split across middle and late) (Figure \ref{fig:rq1_signal_llama}), while Qwen and Gemma show 8/8 languages exclusively in late layers (Figures \ref{fig:rq1_signal_qwen} and \ref{fig:rq1_signal_gemma}). Within late layers, harm precedes harmless peaks in Llama 
(5/8 languages) and Qwen (6/8 languages), suggesting a dominant harm-then-harmless sequential ordering in these models, consistent with a \textit{two-stage late-layer circuit}: first detecting whether content is harmful, then conditioning generation toward harmless responses (Figure \ref{fig:rq1_peaks}). However, Gemma shows the opposite ordering tendency, with only 3/8 languages retaining harm-first ordering (AR, RU, ZH), while 5/8 languages show harmless peaks before harm peaks (DE, EN, HI, ID, VI), suggesting that Gemma conditions generation toward harmless responses prior to fully activating harm-detection circuits. %The mean gap between harm and harmless peaks varies across models (Llama: 5.0 layers, Qwen: 3.0 layers, Gemma: 3.0 layers), with Llama showing the largest separation, partly driven by middle-late  splits in DE (gap=10) and VI (gap=13). Excluding these middle-late splits, the within-late gap in Llama reduces substantially, suggesting the three models are more comparable in late-layer circuit proximity than raw means indicate.
This cross-model reversal indicates that the sequential ordering of harm and harmless signals reflects model-specific alignment procedures rather than a universal architectural property. Notably, across all three LLMs, Vietnamese consistently shows harmless-first ordering (Llama: harmless L14, harm L27; Qwen: harmless L23, harm L26; Gemma: harmless L34, harm L39), the only language exhibiting this pattern cross-model, suggesting language-specific properties of Vietnamese safety alignment 
independent of architecture.
\textcolor{red}{Could be shortened. Also, you show that harmless features are encountered first and then harmful ones. But from this can you conclude the existence of a two-stage late-layer circuit? You will then have to do some probing to make such a conclusion.}
These late-layer peaks and the language-specific ordering motivate whether these harm and harmless circuits are entangled with language identity features, and whether this entanglement varies across the same late layers where safety signals peak, leading towards RQ2.

\begin{tcolorbox}[colback=brown!10, colframe=brown!60!black,
boxrule=0.8pt, arc=4pt]
\textbf{Key Takeaway (RQ1):} Safety signals concentrate progressively in late layers across LLMs and languages, with harm-before-harmless ordering in Llama and Qwen but reversed in Gemma, revealing architecture-dependent safety circuit organization; Vietnamese uniquely exhibits harmless-first ordering across all three models, suggesting language-specific safety alignment properties.
\end{tcolorbox}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}

\begin{tabular}{l cc cc cc}
\toprule
& \multicolumn{2}{c}{\textbf{Llama} (32L)} 
& \multicolumn{2}{c}{\textbf{Qwen} (28L)} 
& \multicolumn{2}{c}{\textbf{Gemma} (42L)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{Lang} 
& \textbf{Harm} & \textbf{Harmless} 
& \textbf{Harm} & \textbf{Harmless} 
& \textbf{Harm} & \textbf{Harmless}  \\
\midrule
AR 
& L27 & L30          
& L24 & L21$^\dagger$  
& L34 & L35          \\

DE 
& L28 & \textbf{L18}$^\dagger$ 
& L23 & L24           
& L39 & L38$^\dagger$           \\

EN 
& \textbf{L19} & L23  
& L21 & L25          
& L40 & L38$^\dagger$           \\

HI 
& L26 & L31           
& L21 & L27           
& L39 & L38$^\dagger$           \\

ID 
& L26 & L30          
& L24 & L27          
& L39 & L37$^\dagger$           \\

RU 
& L29 & L30           
& L24 & L27           
& L30 & L37          \\

VI 
& L27 & \textbf{L14}$^\dagger$ 
& L26 & L23$^\dagger$  
& L39 & L34$^\dagger$  \\

ZH 
& L31 & L31           
& L24 & L25           
& L28 & L33  \\

\midrule

\textit{Both signals late} 
& \multicolumn{2}{c}{5/8 languages} 
& \multicolumn{2}{c}{8/8 languages} 
& \multicolumn{2}{c}{8/8 languages} \\

\textit{Harm-first ordering} 
& \multicolumn{2}{c}{5/8 languages} 
& \multicolumn{2}{c}{6/8 languages} 
& \multicolumn{2}{c}{3/8 languages} \\

\bottomrule
\end{tabular}
\caption{
    Peak layers for harm-associated and harmless-associated SAE features 
    per language and model. 
    Phase boundaries: Llama (early L0--10, middle L11--21, late L22--31), Qwen (early L0--9, middle L10--18, late L19--27), 
    Gemma (early L0--13, middle L14--27, late L28--41).
    \textbf{Bold} = middle-layer peak (exception to dominant late-layer pattern). $\dagger$ = harmless peak precedes harm peak (harmless-first ordering).
}

\label{tab:rq1_peak_layers}
\end{table*}




\subsection{RQ2: Safety-Language Feature Entanglement Across Layers and Architectures}

\textcolor{red}{The word circuit is used often but never defined.}

We measure entanglement between top-5 safety features (harm/harmless) and top-5 language identity features~\textcolor{red}{(I think you did not mention how you identified the language identify features.)} at each layer using two complementary metrics: Jaccard 
overlap (whether safety and language circuits recruit the \textit{same} features) and decoder cosine similarity (whether they write into \textit{overlapping residual stream directions}, regardless of feature identity). Across all models and layer phases, both metrics confirm 
safety-language entanglement; however, decoder cosine consistently reveals stronger coupling than Jaccard, indicating that safety computation is geometrically 
embedded in language-specific subspaces of the residual 
stream, suggesting safety features share residual stream directions with language features even when they do not share same feature IDs.


\begin{comment}
    

\par \noindent \textbf{Early layers: geometric pre-conditioning 
before functional safety computation.}
Early layers show near-zero Jaccard overlap 
(harm: $\leq 0.089$, harmless: $\leq 0.071$ across models) yet non-trivial decoder cosine (Llama harm: $0.156$--$0.236$, 
harmless: $0.152$--$0.271$; Qwen harm: $0.146$--$0.274$, harmless: $0.124$--$0.210$; 
Gemma harm: $0.123$--$0.220$, harmless: $0.090$--$0.174$), \textcolor{red}{(We have to somehow show that these similarities are statistically significant. I mean how do we know if these similarities are high/low?)} indicating that though safety-language rarely shares common feature IDs in early layers, but their safety features are already geometrically positioned 
in language-specific residual stream subspaces before any functional safety computation begins (near-zero safety MI signals in RQ1) (Figures \ref{fig:rq2_line_harm} and \ref{fig:rq2_line_harmless}). %Since early layers carry near-zero safety MI signals (Section 2.1 \ref{}), this constitutes geometric pre-conditioning of safety feature directions before any functional safety computation begins, an architecture-independent finding across all three models. 
However, which safety signal couples to language first varies across architectures: \textit{Jaccard Overlap:} Llama shows harmless-first entanglement in 5/8 languages (DE, EN, ID, RU, ZH) with ID: $0.071$ and ZH: $0.043$ having
highest mean harmless-language Jaccard over early layers, suggesting harmless mechanisms integrate language information earlier than harm-detection (Figure \ref{fig:rq2_jacc_llama}); Qwen shows a balanced split with four languages harm-dominant (ID, DE, EN, RU) and four harmless-dominant (VI, HI, AR, ZH) (Figure \ref{fig:rq2_jacc_qwen}); Gemma shows harm-dominant coupling in 5/8 languages with Russian as the strongly harmless-language overlap exception (Jaccard $= 0.042$) (Figure \ref{fig:rq2_jacc_gemma}). \textit{Decoder Cosine:} Geometrically, EN shows the strongest early harmless coupling in Llama (decoder $= 0.271$) but the weakest in Qwen ($0.124$) and Gemma ($0.087$), while IN and HI show the strongest early harm coupling in Qwen ($0.274$, $0.269$) (Figures \ref{fig:rq2_line_harmless} and \ref{fig:rq2_dec_llama}--\ref{fig:rq2_dec_gemma}), indicating that early safety-language geometric positioning is architecture-dependent even for the same language.
\end{comment}
\textbf{\textcolor{blue}{Writing again with z scores}}
\par \noindent \textbf{Early layers: geometric 
pre-conditioning before functional safety computation.}
Early layers show near-zero Jaccard overlap 
(harm: $\leq 0.089$, harmless: $\leq 0.071$ across 
models) yet non-trivial decoder cosine (Llama harm: 
$0.156$--$0.236$, harmless: $0.152$--$0.271$; Qwen 
harm: $0.146$--$0.274$, harmless: $0.124$--$0.210$; 
Gemma harm: $0.123$--$0.220$, harmless: 
$0.090$--$0.174$), indicating that though 
safety-language rarely shares common feature IDs in 
early layers,  but their safety features are already geometrically 
positioned in language-specific residual stream 
subspaces before any functional safety computation 
begins (near-zero safety MI signals in RQ1) 
(Figures \ref{fig:rq2_line_harm} and 
\ref{fig:rq2_line_harmless}).
Relative to each model's own layer distribution, 
early harm-language decoder cosine is below the model 
average in Llama (mean $z = -0.53$) and Qwen 
(mean $z = -0.59$), confirming that geometric 
entanglement has not yet reached its peak; however, 
Gemma shows above-average harm and harmless 
entanglement already in early layers 
(mean $z = +0.23$ and $+0.53$ respectively), 
showing architecture-specific contrast among LLMs.
In addition, which safety signal couples to language 
first further varies across architectures.
\textit{Jaccard Overlap:} Llama shows harmless-first 
entanglement in 5/8 languages (DE, EN, ID, RU, ZH) 
with ID ($0.071$, $z = +0.89$) and ZH ($0.043$, 
$z = +0.39$) having the highest mean 
harmless-language Jaccard over early layers, 
values substantially above Llama's own harmless 
Jaccard mean ($0.024$), suggesting harmless mechanisms 
integrate language information earlier than 
harm-detection (Figure \ref{fig:rq2_jacc_llama}); 
Qwen shows a balanced split with four languages 
harm-dominant (ID, DE, EN, RU) and four 
harmless-dominant (VI, HI, AR, ZH) 
(Figure \ref{fig:rq2_jacc_qwen}); Gemma shows 
harm-dominant coupling in 5/8 languages with 
Russian as the strongly harmless-language overlap 
exception (Jaccard $= 0.042$, $z = +0.595$) 
(Figure \ref{fig:rq2_jacc_gemma}).
\textit{Decoder Cosine:} Geometrically, EN shows 
the strongest early harmless coupling in Llama 
(decoder $= 0.271$, $z = -0.01$), followed by Qwen ($0.124$, $z = -0.27$) and weakest in Gemma 
($0.087$, $z = +0.67$), while ID and HI show the 
strongest early harm coupling in Qwen ($0.274$, 
$z = -0.62$; $0.269$, $z = -0.85$), notably 
below Qwen's own model average despite being the 
highest early-phase values (Figures \ref{fig:rq2_line_harmless} and 
\ref{fig:rq2_dec_llama}--\ref{fig:rq2_dec_gemma}), indicating that Qwen's 
harm-language geometric entanglement is not
predominantly a early-layer phenomenon, and that early safety-language geometric positioning is architecture-dependent even for the same language.

%\par \noindent \textbf{Middle layers: harm-language entanglement rises while harmless largely disentangles.}
%Across LLMs, harm-language entanglement overall increases in middle layers while harmless-language overlap largely vanishes (Figures~\ref{fig:rq2_line_harm} and \ref{fig:rq2_line_harmless}) with some language- and architecture-specific exceptions, indicating that harm-detection becomes progressively language-conditioned; however, what the model identifies as harmful is processed differently per language. In Llama, DE shows complete zero harm-language Jaccard across L11--L21, the only clean separation window across all languages and models, yet harm-language decoder cosine still rises (DE: $0.179{\to}0.224$, VI: $0.210{\to}0.308$, HI: $0.197{\to}0.274$), confirming geometric entanglement persists even without shared feature IDs (Figures \ref{fig:rq2_jacc_llama} and \ref{fig:rq2_dec_llama}). EN is the only language where harmless-language decoder cosine consistently exceeds harm across all phases (middle: $0.253$ harmless vs $0.192$ harm), suggesting EN safety alignment couples refusal to language identity more persistently than harm-detection. In Qwen, harm-dominance is clear for AR, HI, ID, RU (Jaccard $0.025$--$0.037$, decoder $0.254$--$0.372$), while DE and ZH retain more harmless-language coupling (ZH: Jaccard $0.037$, DE: Jaccard $0.025$), with VI also showing higher harmless decoder cosine than harm (decoder harm $0.246$ vs harmless $0.281$) (Figures \ref{fig:rq2_jacc_qwen} and \ref{fig:rq2_dec_qwen}). In Gemma, both metrics show the sparsest middle entanglement across all models (harm Jaccard $\leq 0.024$, harmless Jaccard $\leq 0.008$; decoder harm $0.135$--$0.196$, harmless $0.049$--$0.099$), confirming that safety features, especially harmless features, disentangle from language identity earlier in Gemma than in Llama or Qwen (Figures \ref{fig:rq2_jacc_gemma} and \ref{fig:rq2_dec_gemma}).

\par \noindent \textbf{Middle layers: harm-language 
entanglement rises while harmless largely disentangles.}
Across LLMs, harm-language entanglement overall 
increases in middle layers while harmless-language 
overlap largely vanishes 
(Figures~\ref{fig:rq2_line_harm} and 
\ref{fig:rq2_line_harmless}) with some language- and 
architecture-specific exceptions; harm-language 
decoder cosine rises from below to near model average 
in Llama (mean $z$: $-0.531 \to -0.011$) and 
above model average in Qwen 
(mean $z$: $-0.590 \to +0.120$), while 
harmless-language decoder cosine falls below model 
average in Llama (mean $z$: $+0.323 \to -0.219$) 
and Gemma (mean $z$: $+0.528 \to -0.380$), 
indicating that harm-detection becomes progressively 
language-conditioned while harmless features begin to 
decouple from language identity; however, what the 
model identifies as harmful is processed differently 
per language.
In Llama, DE shows complete zero harm-language 
Jaccard across L11--L21 ($z = -0.295$, the only 
clean separation window across all languages and 
models), yet harm-language decoder cosine still rises 
(DE: $0.179{\to}0.224$, $z = -0.142$; 
VI: $0.210{\to}0.308$, $z = +0.272$; 
HI: $0.197{\to}0.274$, $z = +0.043$), 
confirming that geometric entanglement persists even 
without shared feature IDs, and is above model 
average for VI while remaining around or below 
average for DE and HI 
(Figures \ref{fig:rq2_jacc_llama} and 
\ref{fig:rq2_dec_llama}).
EN is the only language where harmless-language 
decoder cosine consistently exceeds harm across all 
phases (middle: $0.253$, $z = -0.162$ harmless vs 
$0.192$, $z = +0.078$ harm); notably both values 
are near or below EN's own model average, indicating 
that this inversion reflects EN's globally elevated 
harmless baseline rather than a peak coupling event, 
yet the pattern suggests EN safety alignment couples 
harmless to language identity more persistently than 
harm-detection. In Qwen, harm-dominance is clear for AR, HI, ID, RU 
(Jaccard $0.025$--$0.037$, $z = -0.495$ to $-0.137$; 
decoder $0.254$--$0.372$, $z = -0.220$ to $+0.267$), 
where Jaccard values remain below Qwen's model 
average across all four languages while decoder 
cosine varies --- ID ($z=+0.267$) and RU ($z=+0.056$) reach near or above 
model average geometrically despite minimal 
ID-level overlap.
DE and ZH retain more harmless-language coupling 
(ZH: Jaccard $0.037$, $z = +0.290$; 
DE: Jaccard $0.025$, $z = +0.114$), 
with VI also showing higher harmless decoder cosine 
than harm (harm $0.246$, $z = -0.339$ vs 
harmless $0.281$, $z = +0.090$), where VI harmless 
is at model average while harm is below 
(Figures \ref{fig:rq2_jacc_qwen} and 
\ref{fig:rq2_dec_qwen}).
In Gemma, both metrics show the sparsest middle 
entanglement across all models (harm Jaccard 
$\leq 0.024$, mean $z = -0.011$; harmless Jaccard 
$\leq 0.008$, mean $z = -0.169$; decoder harm 
$0.135$--$0.196$, mean $z = +0.315$; harmless 
$0.049$--$0.099$, mean $z = -0.380$); notably, 
Gemma's harm decoder cosine, despite low absolute 
values, is above Gemma's own model average 
($z = +0.315$) while harmless decoder has already 
fallen substantially below it ($z = -0.380$), 
confirming that in Gemma harmless features 
disentangle from language identity earlier and more 
sharply than harm features, in contrast to Llama 
and Qwen (Figures \ref{fig:rq2_jacc_gemma} and 
\ref{fig:rq2_dec_gemma}). 


%%%% commenting out previous section
\begin{comment}
    
\par \noindent \textbf{Late layers: entanglement peaks in Llama and Qwen but collapses in Gemma.}
In Llama and Qwen, harm-language entanglement peaks 
in late layers where safety MI signals are strongest 
(Section 2.1~\ref{sec:rq1}), confirming near-output harm-detection is maximally language-conditioned ((Figures \ref{fig:rq2_line_harm} and \ref{fig:rq2_line_harmless})). In Llama, HI reaches the highest Jaccard ($0.067$), followed by EN, RU, ZH ($0.044-0.036$). Further, EN shows the lowest late harm decoder cosine similarity 
($0.203$) and highest late harmless decoder ($0.296$); the only language 
where harmless geometrically exceeds harm in late layers, indicating EN harmless features remain more entangled with language features than harm features near output (Figures \ref{fig:rq2_jacc_llama} and \ref{fig:rq2_dec_llama}). In Qwen, late harm entanglement reaches the highest 
values across all models: HI (Jaccard $0.090$, decoder $0.570$), RU ($0.127$, $0.345$), ID ($0.102$, $0.356$), AR ($0.077$, $0.365$); notably, five languages (AR, ID, RU, VI, ZH) also show late harmless decoder cosine ($0.328$--$0.380$), indicating dual geometric entanglement where both harm and harmless features couple to language identity near output, while EN maintains the least entanglement for both metrics (Figures \ref{fig:rq2_jacc_qwen} and \ref{fig:rq2_dec_qwen}). In Gemma, both metrics collapse in late layers: 6/8 languages show Jaccard $0.000$ for both harm and harmless, with only EN and ZH showing isolated residual harm (Jaccard $0.008$ each); yet decoder cosine remains non-zero (harm: $0.077$--$0.129$, harmless: $0.052$--$0.104$), confirming residual geometric alignment persists even when no feature IDs are shared (Figures \ref{fig:rq2_jacc_gemma} and \ref{fig:rq2_dec_gemma}). This late-layer pattern reveals a fundamental architectural divergence: Llama and Qwen implement near-output safety through language-conditioned circuits, while Gemma decouples safety signal strength from 
language entanglement in comparison to others.
\end{comment}



\par \noindent \textbf{Late layers: entanglement peaks 
in Llama and Qwen but collapses in Gemma.}
In Llama and Qwen, harm-language entanglement peaks 
in late layers where safety MI signals are strongest 
(Section~\ref{sec:rq1}), with harm-language decoder 
cosine reaching substantially above each model's own 
layer average (Llama mean $z = +0.596$; Qwen mean 
$z = +0.535$), confirming near-output harm-detection 
is maximally language-conditioned 
(Figures~\ref{fig:rq2_line_harm} and 
\ref{fig:rq2_line_harmless}).
In Llama, HI reaches the highest harm Jaccard 
($0.067$, $z = +0.394$), followed by EN, RU, ZH 
($0.044$--$0.036$; $z = +0.544$, $+0.192$, $+0.192$), 
all above Llama's own Jaccard model average ($z = +0.176$).
Further, EN shows the lowest late harm decoder cosine 
($0.203$, $z = +0.218$) and highest late harmless 
decoder ($0.296$, $z = +0.194$) --- the only language 
where harmless geometrically exceeds harm in late 
layers (Figures~\ref{fig:rq2_jacc_llama} and 
\ref{fig:rq2_dec_llama}).
In contrast, harmless-language decoder cosine remains 
below model average in Llama late layers (mean 
$z = -0.114$), confirming harmless features disentangle 
from language identity toward output while harm features 
couple more strongly.
In Qwen, late harm entanglement reaches the highest 
values across all models and all phases: HI (Jaccard 
$0.090$, $z = +0.762$; decoder $0.570$, $z = +1.123$), 
RU ($0.127$, $z = +0.874$; $0.345$, $z = +0.668$), 
ID ($0.102$, $z = +0.408$; $0.356$, $z = +0.424$), 
AR ($0.077$, $z = +0.545$; $0.365$, $z = +0.742$) --- 
all substantially above or near to Qwen's own model average at both ID ($z = +0.609$) and geometric levels ($z = +0.535$). Notably, five languages (AR, ID, RU, VI, ZH) also 
show late harmless decoder cosine ($0.328$--$0.380$, 
$z = +0.613$ to $+0.971$), indicating dual geometric 
entanglement above model average where both harm and 
harmless features couple to language identity near 
output, while EN maintains the least entanglement for 
both metrics (harm decoder $z = -0.658$; harmless 
decoder $z = -0.757$), the most negative values 
across all languages and phases in Qwen 
(Figures~\ref{fig:rq2_jacc_qwen} and 
\ref{fig:rq2_dec_qwen}).
In Gemma, both metrics collapse in late layers: 6/8 
languages show Jaccard $0.000$ for both harm and 
harmless, with only EN and ZH showing isolated 
residual harm (Jaccard $0.008$ each); harm-language 
decoder cosine and Jaccard fall well below Gemma's 
own model average (harm decoder mean $z = -0.545$; 
harm Jaccard mean $z = -0.236$), while harmless 
decoder also remains below average (mean $z = -0.148$), 
yet decoder cosine remains non-zero (harm: 
$0.077$--$0.129$; harmless: $0.052$--$0.104$), 
confirming residual geometric alignment persists even 
when no feature IDs are shared 
(Figures~\ref{fig:rq2_jacc_gemma} and 
\ref{fig:rq2_dec_gemma}).
This late-layer pattern reveals a fundamental 
architectural divergence: Llama and Qwen implement 
near-output safety through language-conditioned 
circuits (harm decoder mean $z = +0.596$ and 
$+0.535$ respectively), while Gemma decouples safety 
signal strength from language entanglement 
(harm decoder mean $z = -0.545$), the sharpest 
cross-model contrast observed across all phases.



\par \noindent \textbf{Decoder cosine reveals functional 
entanglement beyond what Jaccard captures.}
Across LLMs, decoder cosine substantially exceeds Jaccard overlap (Figures \ref{fig:rq2_line_harm} and \ref{fig:rq2_line_harmless}): HI in Llama ($5\times$: 
Jaccard $0.067$ vs decoder $0.342$), HI in Qwen 
($6\times$: $0.090$ vs $0.570$), and Gemma, where Jaccard 
collapses to $0.000$ yet decoder remains $0.077$--$0.129$.
This systematic gap confirms that safety and language features are \textit{geometrically entangled in the residual stream even when they share no feature IDs}, indicating that safety-language entanglement operates at the level of residual stream subspaces rather than individual feature identities. Safety interventions targeting specific feature IDs may therefore underestimate the true entanglement cost, as the geometric coupling persists independently of ID-level sharing.

\begin{tcolorbox}[colback=brown!10, colframe=brown!60!black,
boxrule=0.8pt, arc=4pt]
\textbf{Key Takeaway (RQ2):} Safety features are geometrically 
entangled with language identity beyond ID-level sharing, with 
harm-language entanglement peaking in late layers for Llama and 
Qwen but collapsing in Gemma despite equivalent safety signals, 
indicating that Gemma implements language-independent safety 
circuits while Llama and Qwen rely on language-conditioned ones. 
English consistently shows the least entanglement across all 
architectures.
\end{tcolorbox}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq2/rq2_line_harm.png}
\caption{Harm$\leftrightarrow$Language entanglement across processing phases for all 8 languages across Llama, Qwen, and Gemma. Solid lines show Jaccard overlap; dashed lines show decoder cosine similarity; shaded area highlights the gap.
}
\label{fig:rq2_line_harm}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq2/rq2_line_harmless.png}
\caption{Harmless$\leftrightarrow$Language entanglement across processing phases for all 8 languages across Llama, Qwen, and Gemma. Solid lines show Jaccard overlap; dashed lines show decoder cosine similarity; shaded area highlights the gap.
}
\label{fig:rq2_line_harmless}
\end{figure*}






\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_mean_lines.png}
\caption{Mean cross-lingual safety feature similarity across processing phases, averaged over language pairs for Llama, Qwen, and Gemma.
}
\label{fig:rq3_mean_lines}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harm_late.png}
\caption{Cross-lingual harm feature similarity for all language pairs in late layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harm_late}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harml_late.png}
\caption{Cross-lingual harmless feature similarity for all language pairs in late layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harml_late}
\end{figure*}

\subsection{Cross-Lingual Safety Feature Sharing}
We extend the entanglement analysis to cross-lingual comparison, computing Jaccard overlap and decoder cosine similarity between top-5 safety features (harm/harmless) across all language pairs, revealing whether the same safety circuits activate across languages or whether each language relies on distinct, non-transferable features.

\par \noindent \textbf{Early layers show minimal cross-lingual sharing across all models.}
Early layers show near-zero Jaccard overlap across all language pairs and models (Llama: $\leq 0.092$, Qwen: $\leq 0.047$, Gemma: $\leq 0.096$), with correspondingly modest decoder cosine (Llama: $\leq 0.172$, Qwen: $\leq 0.128$, Gemma: $\leq 0.186$), 
confirming safety features are almost entirely language-specific before meaningful safety computation begins (Figure \ref{fig:rq3_mean_lines}). In addition, EN also shows the lowest cross-lingual overlap with all other languages across both metrics and all three LLMs (for instance harmless features: $z\leq -1.0$; Figures \ref{fig:rq3_pair_harm_early} and \ref{fig:rq3_pair_harml_early}).

\par \noindent \textbf{Middle layers show substantial cross-lingual convergence.}
Cross-lingual sharing increases sharply in middle layers, with harmless features converging more strongly than harm across LLMs (Figure \ref{fig:rq3_mean_lines}). In Llama, harmless features show the strongest convergence at DE-HI (Jaccard $0.291$, z=$+2.45$; decoder $0.419$, z=$+2.08$), HI-ID (Jaccard 
$0.241$, z=$+1.52$; decoder $0.385$, z=$+1.59$), while harm features remain lower (RU-VI: Jaccard $0.073$, z=$-0.28$; decoder $0.153$, z=$-0.20$) (Figures \ref{fig:rq3_pair_harm_middle} and \ref{fig:rq3_pair_harml_middle}). In Qwen, harm overlap strengthens substantially from earlier layers (AR-ID: Jaccard $0.277$, z=$+1.89$, decoder $0.428$, z=$+1.68$; ID-RU: decoder $0.432$, z=$+1.72$), while harmless reaches higher values (ID-VI: Jaccard $0.413$, z=$+1.22$, decoder $0.542$, z=$+1.00$). In Gemma, harm convergence is strongest among the three 
models (DE-RU: Jaccard $0.314$, z=$+1.20$, decoder $0.494$, z=$+1.08$; VI-ID: Jaccard $0.301$, z=$+1.07$, decoder $0.472$, z=$+0.98$), and harmless features show the highest cross-lingual alignment observed across all models and phases (DE-ZH: Jaccard $0.429$, z=$+1.07$, decoder $0.616$, z=$+0.96$; DE-VI: Jaccard $0.418$, z=$+1.01$, decoder $0.605$ z=$+0.91$; RU-VI: Jaccard $0.404$, z=$+0.91$ decoder $0.557$, z=$+0.70$). Across all models, EN shows near-zero cross-lingual sharing with other language for both signals and both metrics, confirming its architectural isolation extends beyond within-language entanglement to cross-lingual feature sharing (Figures \ref{fig:rq3_pair_harm_middle} and \ref{fig:rq3_pair_harml_middle}).

\par \noindent \textbf{Late layers reveal critical 
architectural divergence in cross-lingual sharing.}
In Llama, late-layer cross-lingual sharing is modest 
for harm (Jaccard $\leq 0.081$, decoder $\leq 0.166$) 
but substantially higher for harmless features (HI-ID: Jaccard $0.144$, z=$+1.85$, decoder $0.275$, z=$+1.87$; HI-VI: Jaccard $0.144$, z=$+1.85$ decoder $0.271$, z=$+1.81$; AR-ID: Jaccard $0.131$, z=$+1.53$, decoder $0.257$, z=$+1.60$), however, lower than middle layers, yet still confirming refusal mechanisms retain more cross-lingual universality than harm detection near output generation (Figures \ref{fig:rq3_pair_harm_late} and \ref{fig:rq3_pair_harml_late}). In Qwen, late-layer sharing reaches the highest values observed across all models and phases for both signals (Figure \ref{fig:rq3_mean_lines}). Harm features show strong cross-lingual coupling (AR-RU: Jaccard $0.515$, z=$+1.81$, decoder $0.684$, z=$+1.56$; ID-VI: Jaccard $0.483$, z=$+1.57$, decoder $0.644$, z=$+1.31$; RU-VI: Jaccard $0.478$, z=$+1.53$, decoder $0.632$, z=$+1.24$), while harmless features show the highest cross-lingual sharing of the entire study (ID-VI: Jaccard $0.598$, z=$+1.21$, decoder $0.752$, z=$+0.94$; VI-ZH: Jaccard $0.561$, z=$+1.03$, decoder $0.749$, z=$+0.93$; AR-ID: Jaccard $0.515$, z=$+0.80$, decoder $0.702$, z=$+0.75$), with a consistent high-sharing cluster of AR, ID, RU, VI, ZH languages. In Gemma, late-layer harm sharing is moderate (ID-ZH: Jaccard $0.299$, z=$+1.14$, decoder $0.452$, z=$+0.95$; ID-VI: Jaccard $0.297$, z=$+1.12$, decoder $0.481$, z=$+1.15$; AR-ID: Jaccard $0.260$, z=$+0.75$, decoder $0.410$, z=$+0.66$) while harmless sharing is lower (ID-ZH: Jaccard $0.208$, z=$+0.89$, decoder $0.358$, z=$+0.94$; AR-ID: Jaccard 
$0.127$, z=$-0.09$, decoder $0.249$, z=$+0.09$), representing a reversal from Llama and Qwen where harmless consistently exceeds harm, suggesting Gemma's late-layer harm circuits are geometrically more shared across languages than its harmless circuits. Across all three models, EN maintains the lowest cross-lingual overlap in late layers (Llama: Jaccard 
$\leq 0.033$, decoder $\leq 0.091$; Qwen: Jaccard 
$\leq 0.125$, decoder $\leq 0.248$; Gemma: Jaccard 
$\leq 0.042$, decoder $\leq 0.093$), confirming EN 
safety features remain geometrically isolated from 
cross-lingual sharing regardless of model or depth (Figures \ref{fig:rq3_pair_harm_late} and \ref{fig:rq3_pair_harml_late}).

\begin{tcolorbox}[colback=brown!10, colframe=brown!60!black,
boxrule=0.8pt, arc=4pt]
\textbf{Key Takeaway (RQ3):} Cross-lingual safety feature sharing 
peaks in middle layers across all models, but diverges in late 
layers: Llama collapses, Qwen continues to increase, reaching the 
highest sharing observed across all models and phases (ID-VI), and Gemma 
shows a reversal where harm plateaus while harmless declines. 
Harmless features are more cross-lingually universal than harm 
in Llama and Qwen, reversed in Gemma late layers, and English 
remains isolated across all architectures.
\end{tcolorbox}

\begin{table}[t]
\centering
\small
%\setlength{\tabcolsep}{5pt}
\scalebox{0.80}{
\begin{tabular}{llccccc}
\toprule
\textbf{Exp.} & \textbf{language} & \textbf{LLM} & \textbf{Strategy} & \textbf{Layer} & 
\textbf{Before} & \textbf{After} \\
\midrule
1a & HI &Llama &abl. harm & L26 & 27.16\% & 8.21\%   \\
1b & HI &Qwen &abl. harm  & L21 & 50.93\% & 19.64\%  \\
1c & HI &Gemma &abl. harm & L39 & 10.86\% & 7.54\%  \\
\midrule
2a & DE &Llama &amp harml & L18 & 28.29\% & 16.15\%  \\
2b & AR &Gemma &amp harm  & L34 &  4.71\% &  8.79\%  \\
\midrule
3a & VI$\rightarrow$ZH &Llama &rep harm & L14 & 26.45\% & 20.14\% \\
3b & VI$\rightarrow$ZH &Qwen &rep harm  & L23 & 19.64\% & 15.64\%  \\
3c & VI$\rightarrow$ZH &Gemma &rep harm & L34 &  9.71\% &  7.86\% \\
\bottomrule
\end{tabular}
}
\caption{Harmful response rates before and after intervention across experiments. [abl: ablate; amp: amplify; harml: harmless; rep: replace].
}
\label{tab:intervention_safety}
\end{table}


\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{plots/intervene/fluency_bars.png}
\caption{
    Fluency class distribution after intervention across 
    all experiments.
    Class~3 (high fluency, red) forms the base; 
    Class~2 (moderate, orange), Class~1 (poor, yellow), and Class~0 (broken, green) stack above.
}
\label{fig:fluency_bars}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{plots/intervene/scatter_fluency_cost.png}
\caption{
    Decoder cosine entanglement (x-axis) vs language 
    identity cost (y-axis), measured as drop in target 
    language ratio after intervention.
}
\label{fig:scatter_lang}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{plots/intervene/scatter_fluency_cost.png}
\caption{
    Decoder cosine entanglement (x-axis) vs fluency 
    degradation (y-axis), measured as percentage of 
    non-Class-3 responses after intervention.
}
\label{fig:scatter_fluency}
\end{figure}






\subsection{Intervention Experiments}

We validate RQ2 and RQ3 through targeted SAE feature interventions, measuring safety change (\% harmful responses), language identity preservation (target language ratio), and fluency degradation 
(\% non-Class-3 responses). Results are in Table~\ref{tab:intervention_safety} and 
Figures~\ref{fig:fluency_bars}--\ref{fig:scatter_lang}.

\paragraph{Exp 1: Harm ablation (HI, all models).}
Ablating top-5 harm features at peak harm layers (Llama L26, Qwen L21, Gemma L39) reduces harmful responses in LLMs (Table~\ref{tab:intervention_safety}). Further, language identity degradation follows the harm-language decoder cosine ordering from RQ2 (Llama: $0.518$, Qwen: $0.541$, 
Gemma: $0.041$, need to add language-specific plots) where the target language ratio drops substantially for Llama and Qwen while being preserved for Gemma, directly confirming that 
higher decoder cosine entanglement predicts higher language identity cost (Figure~\ref{fig:scatter_lang}).
Fluency remains largely preserved, with higher fluency in Gemma and moderate fluency in Llama and Qwen
(Class~3: $76\%$, $79\%$, $95\%$), confirming ablation 
does not completely break generation coherence.

\paragraph{Exp 2a: Harmless amplification (DE, Llama L18).}
Amplifying harmless features at Llama's clean zero-overlap window (L18) reduces harmful responses by $-12.14$ pp with minimal language cost ($\Delta = -0.057$) (Figure \ref{fig:scatter_lang}) and high fluency preservation (Class~3: $92\%$, no Class~0/1) (Figure \ref{fig:scatter_fluency}), consistent with 
the low entanglement ($0.240$) at this layer (Section 2.2 \ref{} need to add language specific plot).

\paragraph{Exp 2b: Harm amplification control (AR, Gemma L34).} Amplifying harm features increases harmful responses ($+4.08$ pp) with near-zero language cost ($\Delta = -0.034$) (Figure \ref{fig:scatter_lang}), confirming the expected direction and Gemma's low entanglement (harm-language decoder cosine: $0.160$) need to add language-specific plots.

\paragraph{Exp 3: Cross-lingual transfer (VI$\rightarrow$ZH).}
Ablating VI harmless features and replacing VI harm features with ZH harm features at random layer 18 tests RQ3 across models with 
different VI-ZH cross-lingual decoder cosine: Llama ($0.028$), Gemma ($0.223$), Qwen ($0.809$).
All three show modest safety improvements ($-6.31$, $-1.85$, $-4.00$ pp) (Table \ref{tab:intervention_safety}). Language identity follows the decoder cosine ordering (Figures \ref{fig:rq3_pair_harm_middle} and \ref{fig:scatter_lang}): Llama preserves VI near-perfectly ($\Delta = -0.004$), Gemma shows a moderate drop ($\Delta = -0.051$), and Qwen 
undergoes a complete language shift ($\Delta = -0.613$, 
ZH appearing at $0.362$), with fluency degrading 
accordingly (Class~3: $98\%$, $90\%$, $64\%$) (Figure \ref{fig:fluency_bars}).
This directly validates RQ3: higher cross-lingual decoder cosine predicts stronger transfer effects.


Across all experiments, decoder cosine scores from RQ2 and RQ3 consistently predict intervention outcomes; higher entanglement produces greater language identity and fluency cost (Figures~\ref{fig:scatter_lang},~\ref{fig:scatter_fluency}), providing a mechanistically grounded account of the safety-language trade-off in multilingual instruction-tuned LLMs.

\begin{tcolorbox}[colback=brown!10, colframe=brown!60!black,
boxrule=0.8pt, arc=4pt]
\textbf{Key Takeaway (Interventions):} Decoder cosine entanglement 
scores from RQ2 and RQ3 consistently predict intervention outcomes: 
harm ablation reduces harmful responses (RQ1) while language identity cost 
scales with entanglement, and cross-lingual feature transfer causes language shift proportional to cross-lingual similarity, providing mechanistic evidence that SAE feature geometry predicts 
the safety-language trade-off in multilingual LLMs.
\end{tcolorbox}

%%%%%% writing as separate sections of Jaccard and decoder but better with 1 section only
\begin{comment}
We measure entanglement between top-5 safety features (harm/harmless)
and top-5 language identity features at each layer using two
complementary metrics: Jaccard overlap (ID-level feature sharing)
and decoder cosine similarity (geometric alignment in the residual
stream).

\subsubsection{Jaccard Overlap Findings}
\par \noindent \textbf{Early layers show divergent entanglement patterns across LLMs.}
As shown in Figure~\ref{fig:rq2_jacc_llama} -- \ref{fig:rq2_jacc_gemma}, early layers reveal divergent patterns across models. Llama shows harmless-first early entanglement in 5/8 languages (DE, EN, ID, RU, ZH) with ID 
(Jaccard $= 0.071$) and ZH (Jaccard $= 0.043$) show the strongest early harmless-language coupling, while harm-language overlaps remain lower across most languages, suggesting harmless mechanisms integrate
language-specific information earlier than harm-detection. Qwen shows a balanced split with four languages harm-dominant (ID, DE, EN, RU) and four harmless-dominant (AR, HI, VI, ZH). Gemma shows harm-dominant early entanglement in 5/8 languages (Figure \ref{fig:rq2_jacc_gemma}),
with Russian as the sole strongly harmless-dominant exception
(Jaccard $= 0.042$). Since early layers carry near-zero safety MI signals (Section 2.1\ref{}), this early entanglement reflects geometric pre-conditioning of safety feature directions in language-specific subspaces before any functional safety computation begins. 
\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_llama.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Llama.}
\label{fig:rq2_jacc_llama}
\end{figure*}
\par \noindent \textbf{Middle layers show harm-dominant shift
across all models, with model-specific variation.} Across all three models, harm-language entanglement increases in comparison to harmless-language overlap in middle layers, indicating that harm-detection becomes progressively 
language-conditioned; what the model identifies as harmful 
is processed differently per language (Figures \ref{fig:rq2_jacc_llama} -- \ref{fig:rq2_jacc_gemma}). In Llama, DE is the only language showing complete 
zero harm-language overlap across all middle layers 
(Jaccard $= 0.000$, L11--L21), a clean separation window. In Qwen, four languages show harm-dominant middle entanglement (AR, HI, ID, RU; harm Jaccard $0.025$--$0.037$), while DE and ZH show the opposite trend with harmless-language overlap 
exceeding harm (DE: harmless $0.025$, harm $0.012$; ZH: harmless 
$0.037$, harm $0.000$). In Gemma, DE shows the highest middle-phase harm entanglement ($0.024$), followed by English, Hindi, 
and Chinese ($0.016$ each), while all harmless-language values collapse to exactly $0.000$ except near zero-value for ZH ($0.008$) in middle layers. 
\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_qwen.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Qwen.}
\label{fig:rq2_jacc_qwen}
\end{figure*}
\par \noindent \textbf{Late layers reveal critical divergence: entanglement intensifies in Llama and Qwen but collapses in Gemma.}
In Llama and Qwen, harm-language entanglement peaks in late 
layers, where safety MI signals are strongest (Section 2.1 \ref{}),
confirming that near-output harm-detection is maximally 
language-conditioned; Llama: HI reaches the highest observed value (Jaccard $= 0.067$), followed by EN ($= 0.044$) and RU, VI, ZH ($0.033$--$0.036$), while harmless-language overlap drops to near-zero across all languages ($\leq 0.011$); Qwen: late-layer harm entanglement reaches the highest values observed across all models and phases: RU ($0.127$), ID ($0.102$), HI ($0.090$), and AR ($0.077$), with harmless language values remaining at or near zero. However, in Gemma, late layers show near-complete collapse: 6/8 languages show exactly $0.000$ for both harm-language and harmless-language, with only EN and ZH showing isolated residual harm values ($0.008$ each) and ZH maintaining a small harmless overlap ($0.008$) throughout all three phases.
This \textit{decoupling of safety signal strength from language 
entanglement} in Gemma reveals that strong safety computation 
near output does not require language-conditioned circuits, where Gemma implements safety through language-independent features while Llama and Qwen rely on language-specific ones, a fundamental difference in how multilingual safety is architecturally realized.

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_gemma.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Gemma.}
\label{fig:rq2_jacc_gemma}
\end{figure*}

\subsubsection{Decoder Cosine Similarity}

While Jaccard overlap measures whether safety and language features 
share the same IDs, decoder cosine captures geometric alignment, whether these features, regardless of their IDs, write into overlapping directions in the residual stream. A key finding across LLMs is that decoder cosine 
substantially exceeds Jaccard overlap at every phase, indicating 
that safety-language entanglement is \textit{functionally stronger 
than mechanistically apparent}: features use different IDs but 
operate in geometrically overlapping subspaces.

\par \noindent \textbf{Early layers show moderate geometric coupling across LLMs.} 


% Custom bibliography entries only
\bibliography{custom}

\appendix


\end{comment}


\bibliography{custom}

\appendix


\section{SAE Training and Evaluation Details}
\label{app:sae}

\subsection{Trained SAEs: Llama-3.1-8B and Qwen2.5-7B}

We train one BatchTopK SAE \citep{bussmann2024batchtopk} per transformer layer on
the post-block residual stream ({resid\_post}), using the
{saprmarks/dictionary\_learning} library \citep{marks2024dictionary}. We strictly follow the training configuration released by \citet{andyrdt_llama, andyrdt_qwen}, including data blend fractions, optimiser settings, and context length.
Table~\ref{tab:sae_config} summarizes the full configuration.

\begin{table}[h]
\centering
\small
\scalebox{0.80}{
\begin{tabular}{lcc}
\toprule
\textbf{Hyperparameter} & \textbf{Llama-3.1-8B} & \textbf{Qwen2.5-7B} \\
\midrule
Architecture              & BatchTopK   & BatchTopK            \\
Hook point                & {resid\_post}   & {resid\_post} \\
Layers covered            & 0--31 (32 total)       & 0--27 (28 total)     \\
Input dimension $d$       & 4{,}096                & 3{,}584              \\
Expansion factor           & $8\times$   &$32\times$ \\
Sparsity $k$              & 64                     & 64                   \\
Learning rate             & $2\times10^{-4}$       & $1\times10^{-4}$     \\
LR warmup steps           & 1{,}000                & 1{,}000              \\
LR decay start            & 80\% of training       & 80\% of training     \\
Training tokens           & 500M                   & 500M                 \\
SAE batch size            & 2{,}048                & 2{,}048              \\
LLM batch size            & 16                      & 16                   \\
LLM context length        & 1{,}024 tokens             & 1{,}024 tokens       \\
\midrule
\multicolumn{3}{l}{\textit{Training data blend}}                         \\
\textsc{lmsys-chat-1m} \citep{zheng2024lmsys}      & 35\% & 35\%        \\
\textsc{pile-uncopyrighted} \citep{gao2020pile}    & 64\% & 64\%        \\
Emergent-misalignment \citep{betley2025emergent}   &  1\% &  1\%        \\
\bottomrule
\end{tabular}
}
\caption{SAE training configuration.}
\label{tab:sae_config}
\end{table}

\noindent


\subsection{Gemma Scope SAEs}

For Gemma-2-9B-IT we use the publicly released {Gemma Scope} PT SAEs
\citep{lieberum2024gemma} ({google/gemma-scope-9b-pt-res}), covering
all 42 residual-stream layers with a dictionary size of 16{,}384 features per layer
under the JumpReLU architecture \citep{rajamanoharan2024jumping}.
\citet{kissane2024transfer} demonstrate that base SAEs transfer faithfully to
instruction-tuned variants, a finding explicitly confirmed for Gemma~2~9B by
\citet{lieberum2024gemma} (Section 4.4 of the Gemma Scope technical report). We therefore apply these pre-trained SAEs directly to Gemma-2-9B-IT activations.

\subsection{SAE Quality Evaluation}
\label{app:sae_eval}

We evaluate SAE reconstruction quality under two settings:
\textbf{out-of-distribution (OOD)}, using 500 documents from the
WikiText-103 test split \citep{merity2017wikitext}, which is different from the training blend; and \textbf{in-distribution (IND)}, using
200 held-out samples drawn from the same training blend
(35\% {lmsys-chat-1m}, 64\% {pile-uncopyrighted},
1\% emergent-misalignment), mirroring the original evaluation
setup of the reference SAE configurations.
Following prior work \citep{marks2024dictionary,galichin2025have}, we report three metrics: {L0}, {variance explained},
and {loss recovered}, with values close to 1.0 indicating near-lossless reconstruction.
Results are reported as the mean $\pm$ standard deviation across all layers in Table \ref{tab:sae_eval}.

\begin{table}
\centering
\scalebox{0.72}{
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Eval} & \textbf{L0} &
\textbf{Var.\ Exp.\ (\%)} & \textbf{Loss Rec.\ (\%)} \\
\midrule
\multirow{2}{*}{Llama-3.1-8B}
  & IND & $68.9 \pm 2.9$ & $77.6 \pm 5.4$ & $98.3 \pm 1.1$ \\
  & OOD & $70.5 \pm 2.5$ & $75.9 \pm 5.5$ & $97.5 \pm 2.1$ \\
\addlinespace
\multirow{2}{*}{Qwen2.5-7B}
  & IND & $64.6 \pm 0.5$ & $86.8 \pm 3.5$ & $99.1 \pm 0.8$ \\
  & OOD & $69.4 \pm 2.9$ & $87.4 \pm 4.6$ & $98.2 \pm 1.8$ \\
\bottomrule
\end{tabular}
}
\caption{SAE quality metrics averaged across all layers (mean $\pm$ std).}
\label{tab:sae_eval}
\end{table}

Both models achieve high loss recovery under both settings, confirming that SAE reconstructions preserve the model's predictive
behavior across all layers.


\section{Dataset}
Please note that, as the tasks of translation and verification of LLM responses involve reviewing potentially harmful or sensitive content, human annotators were informed in advance that the material may contain unsafe or harmful content. They were asked to review the content strictly for the purposes of translation verification and response labeling.
\subsection{Language Translation \label{app_data_trans}} To obtain multilingual prompts for the TechHazardQA dataset \cite{banerjee2025ethical}, we translate the original English questions using Google Translate\footnote{https://translate.google.com/}. To assess translation quality, 100 randomly sampled prompts were reviewed and proofread by the human annotator for all languages. The translations achieved an average agreement rate of approximately $97\%$, confirming the reliability of the translations. 

\begin{figure}
\includegraphics[width=1\linewidth]{plots/judgellm_prompt.png}
\caption{Prompt for Judge LLM for evaluating the safety of LLM-generated responses.}
\label{fig_judgellm}
\end{figure}

\subsection{Dataset Annotation \label{app_data_annot}}
We provide the prompt in Figure \ref{fig_judgellm} to the judge LLM to annotate the response as harmful or harmless. To further minimize bias from any single model, we use three independent LLMs (Llama-3.3-70B\footnote{https://huggingface.co/meta-llama/Llama-3.3-70B-Instruct}, Gemma-3-27B\footnote{https://huggingface.co/google/gemma-3-27b-it}, Qwen3-30B\footnote{https://huggingface.co/Qwen/Qwen3-30B-A3B-Instruct-2507}) as evaluators and adopt a majority-voting scheme to determine the final \textit{harmful/harmless} label for each response. To validate the use of judge LLMs for annotating harmful and harmless labels to the LLM responses across languages, we randomly sampled 100 harmful and 100 harmless responses from each language and compared the final majority-vote judge LLM labels with human annotations, obtaining an average of approximately $94\%$ agreement, supporting the reliability of LLM-based evaluation. This validated setup is then used to label responses across all datasets and languages.


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{plots/fluency_prompt.png}
\caption{
    LLM-as-judge prompt for fluency evaluation of post-intervention responses.
    the final label.
}
\label{fig:fluency_prompt}
\end{figure}


\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_llama.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Llama.}
\label{fig:rq2_jacc_llama}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_qwen.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Qwen.}
\label{fig:rq2_jacc_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_gemma.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Gemma.}
\label{fig:rq2_jacc_gemma}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_llama.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Llama.}
\label{fig:rq2_dec_llama}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_qwen.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Qwen.}
\label{fig:rq2_dec_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_gemma.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Gemma.}
\label{fig:rq2_dec_gemma}
\end{figure*}


\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harm_early.png}
\caption{Cross-lingual harm feature similarity for all language pairs in early layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harm_early}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harml_early.png}
\caption{Cross-lingual harmless feature similarity for all language pairs in early layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harml_early}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harm_middle.png}
\caption{Cross-lingual harm feature similarity for all language pairs in middle layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harm_middle}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harml_middle.png}
\caption{Cross-lingual harmless feature similarity for all language pairs in middle layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harml_middle}
\end{figure*}


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{plots/fluency_prompt.png}
\caption{
    LLM-as-judge prompt for fluency evaluation of post-intervention responses.
    the final label.
}
\label{fig:fluency_prompt}
\end{figure}


\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_normalised_peaks.png}
\caption{
    Normalised peak layer positions (as \% of total model depth) for harm (red) and harmless (blue) signals across 8 languages and 3 LLMs (circle=Llama, square=Qwen, triangle=Gemma). The dashed line marks the approximate late-phase onset ($\sim$68\% depth).
}
\label{fig:rq1_peaks}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_qwen.png}
\caption{
    Harm (red, solid) and harmless (blue, dashed) MI signal strength across layers for all languages 
    (AR, EN, HI, VI) across Qwen. Dotted vertical lines mark phase boundaries (E=early, M=middle, L=late). Filled markers indicate peak layers; shaded region shows the gap between harm and harmless peaks.
}
\label{fig:rq1_signal_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq1/rq1_gemma.png}
\caption{
    Harm (red, solid) and harmless (blue, dashed) MI signal strength across layers for all languages 
    (AR, EN, HI, VI) across Gemma. Dotted vertical lines mark phase boundaries (E=early, M=middle, L=late). Filled markers indicate peak layers; shaded region shows the gap between harm and harmless peaks.
}
\label{fig:rq1_signal_gemma}
\end{figure*}








\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_llama.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Llama.}
\label{fig:rq2_jacc_llama}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_qwen.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Qwen.}
\label{fig:rq2_jacc_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_jaccard_gemma.png}
\caption{Jaccard overlap between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Gemma.}
\label{fig:rq2_jacc_gemma}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_llama.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Llama.}
\label{fig:rq2_dec_llama}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_qwen.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Qwen.}
\label{fig:rq2_dec_qwen}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{plots/rq2/rq2_decoder_gemma.png}
\caption{Decoder cosine similarity between top-5 safety (harm/harmless) and language identity features per language across early, middle, and late layers in Gemma.}
\label{fig:rq2_dec_gemma}
\end{figure*}


\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harm_early.png}
\caption{Cross-lingual harm feature similarity for all language pairs in early layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harm_early}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harml_early.png}
\caption{Cross-lingual harmless feature similarity for all language pairs in early layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harml_early}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harm_middle.png}
\caption{Cross-lingual harm feature similarity for all language pairs in middle layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harm_middle}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{plots/rq3/rq3_pair_ranking_harml_middle.png}
\caption{Cross-lingual harmless feature similarity for all language pairs in middle layers with mean Jaccard and decoder cosine metrics across LLMs.}
\label{fig:rq3_pair_harml_middle}
\end{figure*}


This is an appendix.

\end{document}


